Compactification of Level Maps of Moduli Spaces of Drinfeld Shtukas

We define Drinfeld level structures for Drinfeld shtukas of any rank and show that their moduli spaces are regular and admit finite flat level maps. In particular, the moduli spaces of Drinfeld shtukas with Drinfeld $\Gamma_0(\mathfrak{p}^n)$-level structures provide a good integral model and relative compactification of the moduli space of shtukas with naive $\Gamma_0(\mathfrak{p}^n)$-level defined using shtukas for dilated group schemes.

==> head.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc} 

\usepackage[all,cmtip]{xy}

\usepackage{enumerate}
\usepackage{enumitem}
\usepackage[colorlinks=true,hyperindex,linktocpage=true]{hyperref}
\usepackage[top=1in, left=1in, right=1in, bottom=1in]{geometry}
\usepackage{tikz-cd}

\usepackage{amsmath, amssymb, amsthm}
\usepackage{mathtools}
\usepackage{mathabx}
\usepackage{stmaryrd}

%\usepackage[style=alphabetic, backend=biber]{biblatex}
\usepackage{comment}

\setcounter{tocdepth}{1}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{propDef}[thm]{Proposition + Definition}
\theoremstyle{definition}
\newtheorem{ex}[thm]{Example}
\newtheorem{defnRmk}[thm]{Definition + Remark}
\newtheorem{defn}[thm]{Definition}
\newtheorem{const}[thm]{Construction}
\theoremstyle{remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{warn}[thm]{Warning}

%%%%% Commands

\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\citestacks}[1]{\cite[\href{https://stacks.math.columbia.edu/tag/#1}{Tag #1}]{stacks-project}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		 Symbols

\newcommand{\sets}[1]{\left\{ #1 \right\}}
\newcommand{\set}[2]{\left\{ \, #1 \, \middle \vert \, #2 \, \right\}}
\newcommand{\br}[1]{\left( #1 \right)}
\newcommand{\dbr}[1]{\left( \! \left( #1 \right) \!  \right)}
\newcommand{\sq}[1]{\left[ #1 \right]}
\newcommand{\dsq}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\se}{\subseteq}
\newcommand{\ses}{\subset}
%\newcommand{\se}{\subset} %JHB style
%\newcommand{\es}{\supset} %JHB style
\newcommand{\eqStar}{\overset{(*)}{=}}
\newcommand{\lessStar}{\overset{(*)}{<}}
\newcommand{\und}{\qquad\text{und}\qquad}
\newcommand{\equi}{\quad\Leftrightarrow\quad}
\newcommand{\equiP}[1]{\quad\overset{(#1)}{\Leftrightarrow}\quad}

\newcommand{\ep}{\varepsilon}
\newcommand{\ph}{\varphi}
\newcommand{\sinf}{\set{\infty}}


%arrows
\makeatletter
\newcommand{\xdashrightarrow}[2][]{\ext@arrow 0359\rightarrowfill@@{#1}{#2}}
\def\rightarrowfill@@{\arrowfill@@\relax\relbar\rightarrow}
\def\arrowfill@@#1#2#3#4{%
	$\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
	\relax#4#1
	\xleaders\hbox{$#4#2$}\hfill
	#3$%
}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 		Letters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Cal

\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
%\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}



\newcommand{\OX}{\Oc_X}
\newcommand{\OS}{\Oc_S}
\newcommand{\OXS}{\Oc_{X_S}}
\newcommand{\ODS}[1]{\Oc_{D_{#1,S}}}
\newcommand{\ODnS}{\ODS{n}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BB

\newcommand{\A}{\mathbb{A}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Z}{\mathbb{Z}}

\renewcommand{\H}{\mathbb{H}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{\Fq}{{\F_q}}
\newcommand{\Ga}{\mathbb{G}_a}
\newcommand{\GaL}{\mathbb{G}_{a, \Lc}}
\newcommand{\GaM}{ \mathbb{G}_{a, \Mc}}
\newcommand{\GaR}{\mathbb{G}_{a, R}}
\newcommand{\GaS}{\mathbb{G}_{a, S}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Frac + Bold

\newcommand{\Gf}{\mathfrak{G}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}

\newcommand{\af}{\mathfrak{a}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\ifr}{\mathfrak{i}}
\newcommand{\jf}{\mathfrak{j}}
\newcommand{\mf}{\mathfrak{m}}
\newcommand{\nf}{\mathfrak{n}}
\newcommand{\Pf}{\mathfrak{P}}
\newcommand{\pf}{\mathfrak{p}}
\newcommand{\qf}{\mathfrak{q}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 		Operators


\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\supp}{supp}
\newcommand{\cha}{\gamma}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\ggT}{ggT}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\opp}{opp}
\DeclareMathOperator{\kgV}{kgV}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\Prr}{Pr}
\DeclareMathOperator{\Def}{Def}
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\Res}{Res}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Linear Algebra

\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Adj}{Adj}
\DeclareMathOperator{\Norm}{Norm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Algebraic Geometry

\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spf}{Spf}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Frob}{Frob}
\newcommand{\FrobS}{\Frob_S}
\newcommand{\HHom}{\mathcal{H}om}
\newcommand{\AAut}{\mathcal{A}ut}
\newcommand{\EEnd}{\mathcal{E}nd}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Group stuff


\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Inv}{Inv}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Shtukas

\DeclareMathOperator{\Bun}{Bun}
\DeclareMathOperator{\Sht}{Sht}
\DeclareMathOperator{\Hecke}{Hecke}
\DeclareMathOperator{\Dmod}{Dr-Mod}
\newcommand{\Nilp}{\mathcal{N}ilp}
\newcommand{\Nilpq}{\mathcal{N}ilp_{\Fq\dsq{\zeta}}}
\newcommand{\Ell}{\Ec\ell\ell}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\Dr}{Dr}
\newcommand{\Gam}[1]{\Gamma_0\left(#1\right)}
\newcommand{\GamN}{\Gam{\varpi_{x_0}^n}}
\newcommand{\Gamm}{\Gam{\varpi_{x_0}}}
\newcommand{\ShtGt}{\widetilde{\Sht}'_{\Gamm}}
\newcommand{\Istruct}{$(\ifr^{-1}/A)^{r'}$-structure }
\newcommand{\Istructs}{$(\ifr^{-1}/A)^{r'}$-structures }
\newcommand{\Pstruct}{$(\pf^{-n}/A)^{r'}$-structure }
\newcommand{\Pstructs}{$(\pf^{-n}/A)^{r'}$-structures }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 		Matrices

\newcommand{\matrixRow}[2]{\begin{pmatrix}#1 & #2\end{pmatrix}}
\newcommand{\matrixCol}[2]{\begin{pmatrix}#1 \\ #2\end{pmatrix}}
\newcommand{\abcd}{\begin{pmatrix}a &b\\c &d \end{pmatrix}}
\renewcommand{\matrix}[4]{\begin{pmatrix}#1 & #2\\#3 & #4 \end{pmatrix}}
\newcommand{\sMatrix}[4]{\br{\begin{smallmatrix}#1 & #2\\#3 & #4 \end{smallmatrix}}}
\newcommand{\sVector}[2]{\br{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}}}
\newcommand{\abcdS}{\sMatrix{a}{b}{c}{d}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    	Category Theory

\newcommand{\catname}[1]{\normalfont{\mathbf{#1}}}
\newcommand{\Set}{\catname{Set}}
\newcommand{\Top}{\catname{Top}}
\newcommand{\Div}{\catname{Div}}
\newcommand{\Ab}{\catname{Ab}}
\newcommand{\Grp}{\catname{Grp}}
\newcommand{\Ring}{\catname{Ring}}
\newcommand{\Field}{\catname{Field}}
\newcommand{\Mod}{\catname{Mod}}
\newcommand{\SchFq}{\catname{Sch}/\F_q}
\newcommand{\CC}{\catname{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 			tikz

\newcommand{\tcd}[1]{
\begin{center}
	\begin{tikzcd}
		#1
	\end{tikzcd}
\end{center}
}

